Accelerating Deep Learning by Focusing on the Biggest Losers

This paper introduces Selective-Backprop, a technique that accelerates the training of deep neural networks (DNNs) by prioritizing examples with high loss at each iteration. Selective-Backprop uses the output of a training example's forward pass to decide whether to use that example to compute gradients and update parameters, or to skip immediately to the next example. By reducing the number of computationally-expensive backpropagation steps performed, Selective-Backprop accelerates training. Evaluation on CIFAR10, CIFAR100, and SVHN, across a variety of modern image models, shows that Selective-Backprop converges to target error rates up to 3.5x faster than with standard SGD and between 1.02--1.8x faster than a state-of-the-art importance sampling approach. Further acceleration of 26% can be achieved by using stale forward pass results for selection, thus also skipping forward passes of low priority examples.

==> evaluation_old.tex <==
% !TeX root = ./selective_backprop.tex

\section{Evaluation}
\label{sec:eval}

We evaluate \System{}'s effect on training with several modern image
classification models using four datasets.  Results show that, compared to
\Scan{} and a state-of-the-art importance sampling
approach~\cite{katharopoulos18}, \SB{} reduces wall-clock time needed to reach
a range of target error rates and provides speedups on all four datasets.
Additional analyses show the importance of individual \SB{} characteristics
including selection of high-loss examples as well as robustness to small
amounts of label error.

% (e.g., selection of high-loss examples, dynamic batch selectivity) as well as robustness
% to small amounts of label error.

%We show that \SB{}'s approach, which picks examples proportional to loss, is
%superior to overweighting hard examples, overweighting easy examples, or
%uniformly weighting all.  We also show that \SB{} is robust to small amounts of
%label error.

%\greg{the lead-in paragraph should probably be reorganized, possibly
%as a numbered list of key takeaways or hypotheses.  It kinda seems
%like a list formed by append, right now.}

\vspace{-5px}
\subsection{Experimental Setup}
\label{sec:eval:setup}

%We describe the training setup used to
We train Wide Resnet~\cite{zagoruyko2016} and MobileNetV2~\cite{sandler18}
\angela{add citations} on three datasets using \System{}, \Scan{} as described
in Section~\ref{sec:design}, and our implementation of \Kath{}
\cite{katharopoulos18} using loss as the importance score criteria and no bias
reweighting. We use the training setup specified in \cite{devries2017}, which
includes optimizations including cutout, batch normalization and data
augmentation.

\begin{comment}
\textbf{MNIST.} The MNIST digits database \cite{lecun10} 
consists of 60,000 training images and 10,000 test images, divided into 10 
classes. Each example is a 28x28 pixel image of a handwritten digit. 
We use the training setup from pytorch-examples~\cite{pytorch-examples}. 
We train with an SGD optimizer with $\textit{LR}=0.1$ and $\textit{decay}=0.0005$
and $\textit{batch\_size}=128$.
\end{comment}

\textbf{CIFAR10.} The CIFAR10/100 datasets \cite{krizhevsky09} contain 50,000
training images and 10,000 test images, divided into 10 and 100 classes,
respectively.  Each example is a 32x32 pixel image.  We use
$\textit{batch\_size}=128$. and cutout of length 16.  Training ends after 12
hours.

%three architectures, ResNet18, DenseNet, and MobileNetV2 \cite{he16, huang17, sandler18}

%We use an SGD optimizer with $decay=0.0005$ and an Adam optimizer
%with $decay=0$. 

\textbf{CIFAR100.} We train on CIFAR100 using the setup specified
in~\cite{devries2017}.  We use a static learning rate with $\textit{LR}=0.1$
and an exponentially extrapolated learning rate decay, starting at 0.1 and
decayed by 0.2 at epochs 60, 120 and 160.  We use $\textit{batch\_size}=128$.
and cutout of length 8.  Training ends after 12 hours.

\textbf{SVHN.} SVHN has 604,388 training examples and 26,032 testing examples
of digits taken from Street View images \cite{netzer11}.  The learning rate is
initialized at 0.1 and is gradually decayed by to 0.01 and 0.001 at epochs 5
and 10, respectively.  We use $\textit{batch\_size}=128$. and cutout of length
20.  Training ends after 96 hours.

\begin{figure*}[t]
\begin{minipage}{\textwidth}
        \centering
        \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/eval/staticlr/error-by-backprops-mnist}.pdf}
          \caption{Test error on MNIST}
          \label{fig:static-mnist}
        \end{subfigure}%
        \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/eval/staticlr/error-by-backprops-cifar10}.pdf}
          \caption{Test error for CIFAR10}
          \label{fig:static-cifar10}
        \end{subfigure}%
        \vskip\baselineskip
        \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/eval/staticlr/error-by-backprops-cifar100}.pdf}
          \caption{Test error for CIFAR100}
          \label{fig:static-cifar100}
        \end{subfigure}%
        \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/eval/staticlr/error-by-backprops-svhn}.pdf}
          \caption{Test error for SVHN}
          \label{fig:static-svhn}
        \end{subfigure}%
        \caption{Test error versus training iterations for various datasets with a static learning rate.}
        \label{fig:static-error}
\end{minipage}
% \squeeze{}
% \squeeze{}
\end{figure*}

\begin{table*}[t]
  \centering
\caption{Speedup achieved by \SB{} over \Scan{} and \Kath{} with a static learning rate. Target error rate is the final error rate of \Scan{}. We also train two additional networks on CIFAR10 using \SB{} and confirm that
the trends are consistent across models. Lower error rates achieved with a decayed learning rate are in Table \ref{table:speedup}.}
\small
  \begin{tabular}{
    l
    l
    S[table-text-alignment=center,table-number-alignment=center]
    S[table-text-alignment=center,table-number-alignment=center]
    S[table-text-alignment=center,table-number-alignment=center]
    S[table-text-alignment=center,table-number-alignment=center]
    S[table-text-alignment=center,table-number-alignment=center,table-format=2.0]
  }
                      &                 &             & \multicolumn{1}{l}{\textbf{Target}} & \multicolumn{1}{l}{\textbf{\SB{} Speedup}}    & \multicolumn{1}{l}{\textbf{\SB{} Speedup}} \\
    \textbf{Dataset}  & \textbf{Model}  & \textbf{LR} & \multicolumn{1}{l}{\textbf{Error}}  & \multicolumn{1}{l}{\textbf{over \Scan{}}}     & \multicolumn{1}{l}{\textbf{over \Kath{}}} \\
 \midrule
 MNIST       & LeNet-5       & 0.001 & 1.97\%   & 1.59X     & 1.20X \\
 CIFAR10     & MobileNetV2   & 0.1   & 19.93\%  & 4.17X     & 3.21X  \\
 SVHN        & ResNet18      & 0.1   & 6.26\%   & 2.79X     & 1.82X  \\
 CIFAR100    & Wide ResNet   & 0.1   & 44.4\%   & 2.30X     & 1.55X   \\
 CIFAR10     & DenseNet      & 0.1   & 16.52\%  & 10.26X    &  \\
 CIFAR10     & ResNet18      & 0.1   & 12.2\%   & 1.16X     &  \\
\end{tabular}
% \vspace{-10px}
\label{table:staticlr}
\end{table*}

\vspace{-5px}
\subsection{\System{} Reduces Training Iterations to Target Error Rate}
\label{sec:eval:iterations}

First, we compare the training of \Scan{}, \Kath{}, and \SB{} using
a static learning rate to control for confounding factors.
\System{} reaches final or non-final target error rates
with fewer training iterations (Fig.~\ref{fig:static-error}). 
This can be seen by comparing the x-axis points 
at which lines for each approach reach a particular y-axis value.  
Although the savings depends on the specific target test error
rate chosen, one way to visualize the overall speedup 
across different target accuracy is by comparing the area under
the three curves.  \SB{} reaches nearly every test error value
with significantly fewer training iterations.

\System{} converges faster than \Scan{} by outperforming \Scan{} on challenging examples.  
Figure~\ref{fig:confidences-mobilenets} shows an inverse CDF
of the network's confidence in each ground truth label of the test set; 
the data represents a snapshot in time after training \System{} or \Scan{} 
for 4.7 million and 5 million examples, respectively.  
For each percentile, we plot the target confidence on the y-axis 
(e.g., the 20th percentile of target confidences is 51\%).
The network's classification is the class with the Top-1 confidence (using argmax). 
Therefore, we cannot infer the classification accuracy of an example 
solely from its target confidence (if the target confidence is $<=50\%$).  
In Figure~\ref{fig:accuracy-mobilenets}, we also plot the accuracy of each
percentile of examples.  Generally, examples at lower percentiles are harder
for the network to accurately classify. Using \System{}, the network has higher
confidence and accuracy in these lower percentiles.
For instance, among the examples at the 20th percentile of target
confidences, 29\% of these examples are classified correctly using \SB{} while
only 1\% are classified correctly by \Baseline{}. While this comes at the
cost of confidence in higher percentile examples, test accuracy is not sacrificed.
In fact, \SB{} is able to generalize better across all examples of all
difficulty levels.

\begin{figure*}[t]
%\squeeze{}
\hspace*{\fill}%
\begin{minipage}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth, clip]{figs/neurips19/eval/{target-confidence}.pdf}
    \vspace{-2em}
    \caption{\small{\SB{} has higher confidence in harder examples at the cost of
    confidence in easy examples.}}
    \label{fig:confidences-mobilenets}
\end{minipage}%
    \hfill%
\begin{minipage}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth, clip]{figs/neurips19/eval/{percent-correct}.pdf}
    \vspace{-2em}
    \caption{\small{\SB{} increases accuracy of harder examples, without
    sacrificing accuracy of easy examples.}}
    \label{fig:accuracy-mobilenets}
\end{minipage} 
\hspace*{\fill}%
%\squeeze{}
\end{figure*}

One potential downside of \System{} is that it could increase susceptibility
to noisy labels. However, we show that on SVHN, a dataset known to include
label error~\cite{papernot18}, \System{} still converges faster to almost all
target errors compared to \Baseline{}. We also evaluate \System{} on CIFAR10
with manually corrupted labels. Following the UniformFlip approach in \cite{ren18},
we randomly flip 0.1\% (50 examples), 1\% (500 examples) and 10\% (5000 examples)
of CIFAR10, and train with MobileNetV2. Figure~\ref{fig:cifar10-mobilenet-labelerror} 
shows that \SB{} accelerates training for all three settings.  With 0.1\%
and 1\% of examples randomized, \SB{} reaches \Scan{}'s final test accuracy
with fewer training  iterations. However, with 10\% error, \SB{} increases the final
error by 2.2\%.  So, while \SB{} is robust to modest amounts of label error,
it is most effective on relatively clean, validated datasets.

\begin{figure*}[t]
\begin{minipage}{\textwidth}
        \begin{subfigure}[b]{0.33\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/eval/labelerror/label-error-0.001}.pdf}
          \caption{Test error, 0.01\% shuffled}
          \label{fig:label-error-1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/eval/labelerror/label-error-0.01}.pdf}
          \caption{Test error, 0.1\% shuffled}
          \label{fig:label-error-2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/eval/labelerror/label-error-0.1}.pdf}
          \caption{Test error, 10\% shuffled}
          \label{fig:label-error-3}
        \end{subfigure}%
        \caption{CIFAR10 on MobileNetV2 with label error. Drop in error is caused by learning
        rate decay.}
        \label{fig:cifar10-mobilenet-labelerror}
\end{minipage}
%\squeeze{}
\vspace{-10px}
\end{figure*}
\vspace{-5px}
\subsection{\System{} Reduces Wall-clock Time to Target Error Rate}
\label{sec:eval:fast}

\begin{table*}[t]
  \centering
\caption{Speedups of \System{} and \Kath{} over \Scan{} using a gradually decayed learning rate. Speedups reported assume a 2:1  ratio of latency between backwards and forwards pass.}
\small
  \begin{tabular}{
    l
    l
    l
    l
    l
    l
    l
    %S[table-text-alignment=center,table-number-alignment=center]
    %S[table-text-alignment=center,table-number-alignment=center]
    %S[table-text-alignment=center,table-number-alignment=center]
  }
                    &\multicolumn{1}{l}{\textbf{\Scan{}}} & \multicolumn{1}{l}{\textbf{\SB{}}}  & \multicolumn{1}{l}{\textbf{\Kath{}}}    & \multicolumn{1}{l}{\textbf{Target Error}} & \multicolumn{1}{l}{\textbf{\SB{} Speedup}} & \multicolumn{1}{l}{\textbf{\Kath{} Speedup}} \\
  \textbf{Dataset}  &\multicolumn{1}{l}{\textbf{Error}}   & \multicolumn{1}{l}{\textbf{Error}}        & \multicolumn{1}{l}{\textbf{Error}}            & \multicolumn{1}{l}{\textbf{Range}}        & \multicolumn{1}{l}{\textbf{Range}}    & \multicolumn{1}{l}{\textbf{Range}} \\
 \midrule
 SVHN       & 2.0\%  & 1.9\%  & 2.1\%  & 5--15\% & 1.0--3.1X    & 0.5--2.0X \\
 CIFAR10    & 7.2\%  & 5.6\%  & 6.6\%  & 10-20\% & 1.2--4.4X    & 0.6--1.8X \\
 CIFAR100   & 18.8\% & 20.0\% & 37.6\% & 40-50\% & 1.0--1.6X    & 0.4--0.7X \\
\end{tabular}
\label{table:speedup}
%\squeeze{}
\end{table*}

\begin{comment}
\begin{table*}[t]
  \centering
\caption{Speedups of \System{} over \Scan{} using a gradually decayed learning rate. Target errors chosen to be 10 lowest errors achieved by baseline. Speedups reported assume either a 2:1 or 10:1 ratio of latency between backwards and forwards pass.}
\small
  \begin{tabular}{
    l
    l
    l
    l
    l
    %S[table-text-alignment=center,table-number-alignment=center]
    %S[table-text-alignment=center,table-number-alignment=center]
    %S[table-text-alignment=center,table-number-alignment=center]
  }
                    &                 & \multicolumn{1}{l}{\textbf{Target Error}} & \multicolumn{1}{l}{\textbf{\SB{} Speedup}} & \multicolumn{1}{l}{\textbf{\SB{} Speedup}}     \\ %& \multicolumn{1}{l}{\textbf{\Kath{} Speedup}} \\
  \textbf{Dataset}  & \textbf{Model}  & \multicolumn{1}{l}{\textbf{Range}}        & \multicolumn{1}{l}{\textbf{Range (2x)}}    & \multicolumn{1}{l}{\textbf{Range (10x)}}          \\ %& \multicolumn{1}{l}{\textbf{Range}} \\
 \midrule
 MNIST       & LeNet-5       & \ \ 4--13\%  & 0.3--1.4X    & 0.4--2.0X \\
 CIFAR10     & MobileNetV2   & 11--21\% & 1.6--4.4X    & 2.3--6.7X \\
 CIFAR100    & Wide ResNet   & 11--21\% & 2.0--2.7X    & 3.1--4.1X \\
 SVHN        & ResNet18      & \ \ 4--14\%  & 0.8--3.1X    & 1.0--4.2X \\
\end{tabular}
\label{table:speedup-old}
%\squeeze{}
\end{table*}
\end{comment}

Although \SB{} reduces training iterations, it does not skip forward passes. 
Therefore, \SB{}'s wall-clock speedup depends on the ratio of 
time taken for the backward pass to that for the forward pass.
In practice, this ratio depends heavily on the training setup. As noted in~\cite{convbenchmarks} 
and confirmed in Fig.~\ref{fig:asymmetry}, on current GPUs, calculating
the backward pass typically takes two times as long as  the forward pass. 
With hardware accelerators such as TPUs, we could expect even 10X~\cite{jouppi17},
further increasing \SB{}'s training time benefit. To analyze the speedup attained by
\SB{}, we measure the number of forward and backward passes needed to achieve a
particular target error rate.  We then calculate the speedup of \SB{} and \Kath{}
assuming a 2:1 cost ratio between the forward and backward pass.

We report the speedup achieved by \SB{} over \Scan{} and \Kath{} to the final
error rate of \Scan{} when training with a static learning rate
(Table~\ref{table:staticlr}). Compared to \Scan{}, \System{} accelerates
training by \BaselineSpeedupRange{}, even on modern hardware, without the
use of inference accelerators or memoization. \System{} also achieves a
\KathSpeedupRange{} speedup over \Kath{}. We train \System{} and \Scan{}
using MobilenetV2 on two additional networks to show that the same speedup trends
hold across different networks (Table~\ref{table:staticlr}). We include the training curves
in the supplementary material.

In order to evaluate speedups to competitive target error rates, we introduce
a learning rate scheduler into training, as described in Section~\ref{sec:eval:setup}.
For each dataset, we choose 10 target errors that are reached by all three approaches.
We report the final error for \Scan{}, \SB{} and \Kath{} and the range of speedups over
\Scan{} achieved by \SB{} and \Kath{} for these target errors (Table~\ref{table:speedup}).
The training curves and the speedups for each target error are included in the
supplementary material. Our results show that \SB{} reduces wall-clock time
for a range of competitive target error rates, even compared to \Kath{}. \SB{} and \Kath{}
achieve similar final error rates to \Baseline{}, with the exception of \Kath{}
on CIFAR100. We confirm that this is a comparable final error rate reported for CIFAR100
in ~\cite{katharopoulos18}. 

\textbf{Future work.} Determining a comparable learning rate schedule when applying a sampling
method like \SB{} is an open question that we leave for future work. We expect that the final error rates between \Scan{} and
\SB{} would be even closer by optimizing the learning rate schedule for both. To further reduce
wall-clock time using \SB{}, we could tailor the \SB{} algorithm to reduce forward passes by,
e.g., memoizing particularly easy examples or by adaptively tuning selection probabilities as
training converges. Well-known techniques, such as running the forward passes in parallel
and using reduced precision, can further reduce wall-clock time. We also leave this analysis to future work.

\begin{figure*}[t]
\begin{minipage}{\textwidth}
        \begin{subfigure}[b]{0.3\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/motivation/asymmetry/k20-mobilenetv2}.pdf}
          \caption{NVIDIA Tesla K20}
          \label{fig:asymmetry-k20}
        \end{subfigure}%
        \begin{subfigure}[b]{0.3\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/motivation/asymmetry/gtx1070-mobilenetv2}.pdf}
          \caption{NVIDIA GeForce GTX-1070}
          \label{fig:asymmetry-gtx}
        \end{subfigure}%
        \begin{subfigure}[b]{0.3\textwidth}
          \includegraphics[width=\linewidth]{{figs/neurips19/motivation/asymmetry/titanv-mobilenetv2}.pdf}
          \caption{NVIDIA TitanV}
          \label{fig:asymmetry-titanv}
        \end{subfigure}%
        \caption{Breakdown of processing time per batch while training MobileNetV2 with \Scan{}.}
        \label{fig:asymmetry}
\end{minipage}
%\squeeze{}
\vspace{-10px}
\end{figure*}

\begin{comment}
asymmetry between the forwards and backwards pass.
Table~\ref{table:speedup} reports on the speedup \SB{} achieves compared to
\Scan{} for a range of target errors.

As indicated by the first vertical line, using \System{} has little-to-no
impact for two cases and a moderate ($<$20\%) slowdown for the third;
recall that it provides better final error rate in exchange.
But, with greater ratios, \System{} can also reduce wall-clock time for training.
For example, With software acceleration using
techniques such as reduced precision, quantization, fused kernels and
sparsification, there are reports of an order of magnitude speedups of
inference (denoted by the "Estimated Ratio after SW Optimization"
line)~\cite{tensorrt17, tensorrt4}.
As indicated by the second vertical line, this would result in
10--35\% speedup in training time (in addition to the final error rate benefits).
With hardware acceleration, for instance
using TPUs, the ratio could be even higher~\cite{jouppi17}, 
further increasing \SB{}'s training time benefit.
%. Under such conditions,
%\System{} will reduce training time. 
\end{comment}

\begin{comment}
In \System{}, we do not use a static selectivity. Instead of comparing an
example to others in a batch, we independently determine whether an example
should be used for training. This means that the frequency an example is
backpropped is true to it's likelihood of backprop. That is, an example which
has a 20\% likelihood of being backpropped will be backpropped once every five
epochs, regardless of the probability of other examples.  We compare
Approaches which use a predetermined selectivity \cite{katharopolous18} compare
the relative scores of examples to determine which examples to use for
training.  
\end{comment}

\begin{comment}
\textbf{Improving wall-clock time.} The wall-clock time needed to achieve a
target accuracy depends on the ratio of time spent in the forward and backward
pass. As inference accelerators improve, we expect the backward pass to
increasingly dominate the time of the forward pass. However, the actual ratio
depends on the hardware used. To use \System{} to improve wall-clock time, we
must first tune \SampleMin{} to be the right amount of filtering so as to gain
the benefits of sampling, without incurring too many extra forward passes.
Automatically tuning the \SampleMin{} is an open question left to future work.
\end{comment}

%\subsection{\System{} can cause overfitting to bad examples}

%\subsection{Example images from datasets}


\begin{comment}
Table~\ref{table:error-reduced} summarizes the error rates achieved using \SB{}
and \Scan{}.  \SB{} finds more generalized solutions (with lower test error)
for MNIST (Fig.~\ref{fig:error-mnist}) and CIFAR10
(Fig.~\ref{fig:mobilenet-error}) and achieves comparable final error rates for
CIFAR100 (Fig.~\ref{fig:error-cifar100}) and SVHN (Fig.~\ref{fig:error-svhn}).
Figure~\ref{fig:mobilenet-ratio} \footnote{Ratios for \Scan{} and \Random{} are
always 1, and not visible} shows that the ratio of examples that are
backpropped by \SB{} over time is dependent on the network's loss
(Fig.~\ref{fig:mobilenet-loss}).  As the network converges, \System{} filters
more examples.  \System{} reaches a final error rate of 7.22\%, decreasing test
error compared to \Scan{} by 22\% (Fig.~\ref{fig:mobilenet-error}). For
comparison, we show that randomly sampling 10\% examples leads to slower
learning and higher final test error.  We also show that these trends hold
across diverse network architectures, DenseNet (Fig.~\ref{fig:error-densenet})
and ResNet18 (Fig.~\ref{fig:error-resnet}).

\begin{figure*}[t]
\begin{minipage}{\textwidth}
  \hspace*{\fill}%
        \begin{subfigure}[t]{0.33\textwidth}
          \includegraphics[width=\linewidth]{{figs/error/densenet-0.1}.pdf}
          \caption{Test error for DenseNet}
          \label{fig:error-densenet}
        \end{subfigure}%
        \hfill%
        \begin{subfigure}[t]{0.33\textwidth}
          \includegraphics[width=\linewidth]{{figs/error/resnet-0.1}.pdf}
          \caption{Test error for ResNet18}
          \label{fig:error-resnet}
        \end{subfigure}%
  \hspace*{\fill}%
\end{minipage}
\caption{CIFAR10 with DenseNet and ResNet18.}
\vspace{1em}
%\squeeze{}
\end{figure*}

\textbf{Benefit of self-pacing.} As the network converges, \System{}'s
selectivity organically increases, filtering more and more examples.  This
self-pacing is a significant advantage over an approach that uses a constant,
pre-determined selectivity.  Figure~\ref{fig:kath} compares \System{} to
\Kath{}, our own implementation of the technique described in
\cite{katharopoulos18}, a state-of-the-art technique with a \textit{constant}
selectivity. In \Kath{}, we perform a forward pass on 1024 candidate examples
and sample 128 with replacement, where each example's probability is its
normalized cross-entropy loss. We reweight the loss of each chosen example
proportional to its sampling probability.  We see that \Kath{} outperforms
\KathUniform{}, the baseline from \cite{katharopoulos18} in which training
examples are sampled from a uniform distribution. \KathBiased{} (a version of
\Kath{} that does not reweight losses) outperforms \Kath{}.

\System{} trains faster than \KathBiased{} because of its self-pacing. \SB{}
backprops most examples early on in training, but it becomes more selective
over time. By contrast, \Kath{}, \KathBiased{} and \KathUniform{} always
backprop 1/8 of the examples.  Further, \System{} processes the dataset
sequentially (``scan'') rather than sampling with replacement.
\cite{katharopoulos18} has a warm-up phase that turns on sampling only once it
is expected to reduce the variance by a threshold.  This warm-up period
requires tuning a hyperparameter (warm-up duration), however, and does not pace the selectivity
continuously and dynamically over time.  \giulio{Note: The current way we
  compute probabilities naively relies on the behavior/shape of L2 loss. You
could imagine adding a "dampening" hyperparameter that makes the probability
closer to uniform, or using a different distance metric.}

\mk{The graphs show lots of noise of the Kath18 experiments, but there is no explanation
of that in the text.}

\begin{figure*}[t]
%\squeeze{}
\hspace*{\fill}%
\begin{minipage}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth, clip]{figs/error/{kath}.pdf}
    \vspace{-2em}
    \caption{Comparison against Katharopoulos18 on CIFAR10 with MobileNetV2}
    \label{fig:kath}
\end{minipage}%
    \hfill%
\begin{minipage}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth]{figs/error/{probs-mobilenetv2-0.1}.pdf}
    \vspace{-2em}
    \caption{ \SB{} vs. using only the hardest examples per minibatch,
    only the easiest, and the uniform distribution. (Still running).}
    \label{fig:probs-mobilenetv2}
\end{minipage} 
\hspace*{\fill}%
%\squeeze{}
\end{figure*}

\textbf{Benefit of loss-proportional probability.}
\System{} scales the
probability of choosing an example proportional to its loss.
Figure~\ref{fig:probs-mobilenetv2} compares \SB{}
to three alternative approaches: training with mostly hard examples (Top-K), mostly
easy examples (Low-K), or a uniform sampling of both (Random-K). In Top-K and
Low-K we choose the 13 out of 128 examples with the highest and lowest losses,
respectively. Random-K is a control, sampling a random 13 out of 128
examples to train. Like \SB{}, we backprop our selected examples as
minibatches of size 128.

The results match our expectations.  Focusing on easy examples (Low-K)
fails to learn.  Top-K, while better, is still worse than
Random-K (which behaves like Baseline), because it fails to sufficiently learn
the common cases.
%In Figure~\ref{fig:probs-mobilenetv2}, we show that the best performance comes
%from sampling proportional to loss.
Sampling proportional to loss (\System{}) performs best,
emphasizing the hardest examples while ensuring thorough learning of
the simpler examples.

\textbf{Benefit of not reweighting.} By disproportionally training on the
examples with higher loss, \System{} guides the network toward a more robust
solution that provides better generalization and lower final error.
Figure~\ref{fig:confidences-mobilenets} shows a CDF of the network's confidence
in each ground truth label of the test set; the data represents a snapshot in
time after training \System{} or \Scan{} for 4.7 million and 5 million
examples, respectively.  For each percentile, we plot the target confidence on
the y-axis (e.g., the 20th percentile of target confidences is 44\%).  \mk{This
sentence is passive voice, but also could be clearer...can someone take a shot
at improving?} The network's classification is the class with the Top-1
confidence (using argmax).  Therefore, we cannot infer the classification
accuracy of an example solely from its target confidence (if the target
confidence is $<=50\%$).  Therefore, in Figure~\ref{fig:accuracy-mobilenets} we
also plot the accuracy of each percentile of examples.  For instance, among the
examples at the 20th percentile of target confidences, 20\% of these examples
are classified correctly using \SB{}.  Generally, examples at lower percentiles
are harder for the network to accurately classify.  Using \System{}, the
network has higher confidence and accuracy in these lower percentiles. \SB{}
does not sacrifice classification accuracy at higher percentiles, but also
generalizes better across all examples of all difficulty levels.

\end{comment}

